Using competency questions to select optimal clustering structures for residential energy consumption patterns

During cluster analysis domain experts and visual analysis are frequently relied on to identify the optimal clustering structure. This process tends to be adhoc, subjective and difficult to reproduce. This work shows how competency questions can be used to formalise expert knowledge and application requirements for context specific evaluation of a clustering application in the residential energy consumption sector.

==> sections/clustering_experiments.tex <==
\section{Setup of Clustering Experiments}

The objective of the load profile clustering experiments is the selection of the experiment that produces the set of clusters $k^{(i)}$ that symbolise the best RDLPs $R^{(i)}$ for $X$, so that the RDLPs can be used to generate customer archetypes. The clustering process was set up as a typical data processing pipeline, using hourly daily load profiles from DELMH as input. Depending on the experiment, different pre-processing steps were performed. These include the selection of a pre-binning by average monthly consumption (AMC) or integral k-means, and retaining or dropping zero values. Each of the experiments was run with four different normalisation algorithms, as well as no normalisation. Algorithms were initialised with different sets of parameter values to generate cluster sets with a range of membership sizes. Details on the algorithms, normalisation and pre-binning are provided in Appendix \ref{appendixb}. 

\subsection{Quantitative Metrics and CI Score}

To ease the quantitative evaluation process and allow for comparison across metrics, Mean Index Adequacy (MIA), Davies-Bouldin Index (DBI) and the Silhouette Index were combined into a Combined Index (CI) score. $Ix$ is an interim score that computes the product of the DBI, MIA and inverse Silhouette Index. The CI is the log of the weighted sum of $Ix$ across all experiment bins. A lower CI is desirable and an indication of a better clustering structure. The logarithmic relationship between $Ix$ and the CI means that the CI is negative when $Ix$ is between 0 and 1, 0 when $Ix = 1$ and greater than 0 otherwise. For experiments with pre-binning, the experiment with the lowest $Ix$ score in each bin is selected, as it represents the best clustering structure for that bin. For experiments without pre-binning, $bins = 1$ and $N_{bin} = N_{total}$.
